Cultural Transmission, Property Rights, and Treatment of the Elderly

We examine how production and the development of property rights interact with cultural transmission to shape the treatment of the elderly across societies. Our model posits that respect for the elderly arises endogenously: parents invest in cultivating cultural values in their children, who later reciprocate in proportion to this investment. We show that this model is functionally equivalent to one in which cultural goods are transferred by the elderly. We focus on the distinct roles of property rights, finding that while insecure output rights may promote elderly welfare, secure rights over productive resources can have comparable benefits. The model reveals a nonlinear relationship between cultural sophistication, property rights, and economic factors such as the capital and land intensity of production, driving variations in elderly well-being across societies. Finally, we consider how the model suggests demographic, technological, and policy changes influence elderly well-being across the spectrum of development.

==> expprodvars.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{cccccc}}
\toprule
                    &            &        Mean&          SD&         Min&         Max&           N\\
\midrule
Male rites of initiation&            &        2.40&        1.00&           0&           3&          25\\
Female rites of initiation&            &        1.90&        0.94&           0&           3&          21\\
Males marriage rites&            &        2.77&        0.43&           2&           3&          31\\
Females marriage rites&            &        2.43&        0.60&           1&           3&          21\\
Males funereal rites&            &        2.60&        0.76&           0&           3&          25\\
Females funereal rites&            &        2.54&        0.51&           2&           3&          26\\
Male priesthood     &            &        2.86&        0.36&           2&           3&          35\\
Female priesthood   &            &        1.85&        0.69&           0&           3&          13\\
Male shamans        &            &        2.86&        0.39&           1&           3&          59\\
Female shamans      &            &        2.49&        0.69&           0&           3&          47\\
Male decorators     &            &        2.33&        0.58&           2&           3&           3\\
Female decorators   &            &        2.67&        0.50&           2&           3&           9\\
\bottomrule
\end{tabular}
}

